XRBench: An Extended Reality (XR) Machine Learning Benchmark Suite for the Metaverse

Real-time multi-task multi-model (MTMM) workloads, a new form of deep learning inference workloads, are emerging for applications areas like extended reality (XR) to support metaverse use cases. These workloads combine user interactivity with computationally complex machine learning (ML) activities. Compared to standard ML applications, these ML workloads present unique difficulties and constraints. Real-time MTMM workloads impose heterogeneity and concurrency requirements on future ML systems and devices, necessitating the development of new capabilities. This paper begins with a discussion of the various characteristics of these real-time MTMM ML workloads and presents an ontology for evaluating the performance of future ML hardware for XR systems. Next, we present XRBENCH, a collection of MTMM ML tasks, models, and usage scenarios that execute these models in three representative ways: cascaded, concurrent, and cascaded-concurrent for XR use cases. Finally, we emphasize the need for new metrics that capture the requirements properly. We hope that our work will stimulate research and lead to the development of a new generation of ML systems for XR use cases. XRBench is available as an open-source project: https://github.com/XRBench

==> AE_SubSections/09_Methodology.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Methodology}

Submission, reviewing and badging methodology:

\begin{itemize}
  \item \url{http://cTuning.org/ae/submission-20190109.html}
  \item \url{http://cTuning.org/ae/reviewing-20190109.html}
  \item \url{https://www.acm.org/publications/policies/artifact-review-badging}
\end{itemize}


==> formulae/frm_ValidSchedule.tex <==
\begin{BOX}[ht]
\centering

\fbox{
 \addtolength{\linewidth}{-2\fboxsep}%
 \addtolength{\linewidth}{-2\fboxrule}%
\begin{minipage}{\linewidth}

\insertFormula{Dependency Condition}
{-1.5}
{
\forall h_1, h_2 \in HW, \mu_{i} \in Dep_{\mu_{j}}, T_{end}(\mu_{i}, h_1) < T_{start}(\mu_{j}, h_2)
}
%%%%%%%%%%%%%%%%%%%%%%
\insertFormula{Hardware Occupancy Condition}
{-3}
{
&\forall \mu_{1}, \mu_{2} \in M, \\ 
&(T_{end}(\mu_{1},h) \leq T_{start}(\mu_{2},h)) \lor (T_{end}(\mu_{2},h) \leq T_{start}(\mu_{1},h)) \\ 
&\text{where } T_{end}(h,\mu) = \infty \land T_{start}(h,\mu) = 0 \text{ if } \mu \text{ is not mapped on } h
}
\end{minipage}
}
\caption{Conditions for a valid schedule}
\end{BOX}


==> formulae/frm_XRBenchScore.tex <==

\begin{BOX}[ht]
\centering


\fbox{
 \addtolength{\linewidth}{-2\fboxsep}%
 \addtolength{\linewidth}{-2\fboxrule}%
\begin{minipage}{\linewidth}
%%%%%%%%%%%%%%%%%%%%
\insertFormula{Inference-wise Score ($Score_{inf}(IR)$)}
{-1.5}
{
Score_{inf}(IR) = &RtScore(IR) \times EnScore(IR) \\  
&\times MqScore(IR)
}
%%%%%%%%%%%%%%%%%%%%
\insertFormula{Usage Scenario Score ($Score_{scn}(\theta)$)}
{-1}
{
Score_{scn}(\theta) = 
\sum_{j=1}^{NumFrm(\mu)}{} 
\frac{Score_{inf}(IR)\times QoEScore(\mu)}{NumFrm(\mu) \times |\theta|}
}
%%%%%%%%%%%%%%%%%%%%
\insertFormula{XRBench Score ($Score_{bench}$)}
{-2}
{
Score_{bench} = \frac{\sum_{\theta \in \Omega}{Score_{scn}(\theta)}}{|\Omega|}
}
\end{minipage}
}
\vspace{-3mm}
\caption{XRBench Score}
\label{box:xrbench_score}
\vspace{-6mm}
\end{BOX}


==> notes/formulation.tex <==
(v1)
Inputs: 
N: Number of models in the workload
T0: start time, T0 >= 0
W: Workload list, W = {(mi, fi, di) | 0 <= i < n}
Td: Data arrival time (relative to the start time) for each model, Td = { Tdi | 0 <= i < n }
Dp: Model dependency, Dp = {(mi, mj) | i != j }
S: Schedule S = {(mi, Tsi, Tfi) | 0 <= i < n}, where Tsi and Tfi are start and completion time of model mi.

(Body to be defined)

Output:
Sl: Score (latency side)


\HK{There are two possible formulations. Doing scheduling within the scoring metric (i.e., ensure the best schedule when we compute scores) or taking a schedule as an input. This version take the latter approach. This allows people to develop their own scheduler.} 

\HK{As the workloads are repeated over time (e.g., we continuously run hand tracking while a user is playing a game), we can decide how to run next iterations. There are two possibilities; (1) start next run as soon as the previous run finishes (2) wait until designated next run start time (e.g., if we finish all the models in 0.7 seconds, we wait until 1 second and launch the next run then). (2) would make more sense for us as data arrival time is based on constant FPS. This also makes the problem simpler.}

(v2)
Inputs: 
N: Number of models in the workload
T0: start time, T0 >= 0
W: Workload list, W = {(mi, fi, di) | 0 <= i < n}
Td: Data arrival time (relative to the start time) for each model, Td = { Tdi | 0 <= i < n }
M: Memory size
Dp: Model dependency, Dp = {(mi, mj) | i != j }
S: Schedule S = {(mi, Tsi, Tfi) | 0 <= i < n}, where Tsi and Tfi are start and completion time of model mi.

(Body to be defined)

Output:
Sl: Score (latency side)


Difference from v1: check memory footprint as well. If the processing time is not fast enough to clear memory space for other incoming data, penalize the system.


==> sections/04_ScoreFormulation.tex <==
\section{Problem Formulation}
\label{sec:problem_formulation}
%\HK{TODO (Minor): Improve the notations to be more concise and clear. (e.g., $Dep_{\mu}$ could be $Dep(\mu)$)}



\begin{definition}
\textbf{Input Data Stream} \\
The input data stream $I$ is defined as follows:
$$St_{input} = \{(inSrc, SR, L_{init}, Jt)$$
$$~|~inSrc, SR, L_{init}, Jt \in \mathbb{N} \}$$ 
\label{def:input_data_stream}
\end{definition}
~\autoref{box:base_defs}
~\autoref{def:input_data_stream} formulates the input stream description in~\autoref{tab:input_sources}. The $inSrc$ refers to the input source identifier. $SR$ refers to the streaming rate (FPS). $L_{init}$ refers to the initial latency of each input stream, and $Jt$ refers to the maximum jitter in milliseconds.

\begin{definition}
\textbf{Unit models} \\
The set of unit models $M$ is defined as follows:
$$ M = \{ (M_{ID}, inSrc, ds, goal) ~|~ M_{ID}, ds \in str $$
$$\wedge inSrc \in \mathbb{N} \wedge goal = (metric_{ID}, metric_{targ})\} $$
\label{def:unit_models}
\end{definition}

~\autoref{def:usage_scenario} defines the set of unit models. $\mu$ refers to a unit model (i.e., an element of $M$), $M_{ID}$ refers to the model ID, $inSrc$ refers to the input source ID in~\autoref{def:input_data_stream}, $ds$ refers to the data set, $goal$ is a tuple of the target metric ID in string and the $target\_value$ of the metric in a floating point number. Based on the definition of $D$, we define the usage scenario as follows:

%\newtheorem{definition}{Definition}
\begin{definition}
\textbf{Usage Scenario} \\
Given a set of unit models $M$ to be included to usage scenarios, a usage scenario $\theta$ is defined as follows:
$$\theta = \{(\mu, Dep_{\mu}, \gamma)~|~\mu \in M \wedge \gamma \geq 0 \wedge Dep_{\mu} \subset M \} $$
where $\gamma$ is an integer.
\label{def:usage_scenario}
\end{definition}

In \autoref{def:usage_scenario}, $Dep_{\mu}$ defines the model granularity dependency on $\mu$, which lists up the set of models $\mu$ depends on. When we have multiple pipelines for the same model (e.g., two eye tracking model runs for each eye), we include multiple instances of the same model within $\theta$, with different input sources if necessary. With~\autoref{def:usage_scenario}, we can define the benchmark suite using as follows.

\begin{definition}
\textbf{Benchmark Suite} \\
Given a set of usage scenarios $\Theta$, a real-time \abbrvWorkload{} benchmark suite  $\Omega$ is defined as follows: 
$$
\Omega = \{\theta~|~\theta \in \Theta \} 
$$
\label{def:becnmark_suite}
\end{definition}

The~\autoref{def:becnmark_suite} shows that a real-time \abbrvWorkload{} benchmark is a collection of usage scenarios as described in~\autoref{tab:usage_scenario_processing_rates}. Now we formulated the benchmark suite. We define some additional concepts for defining the scoring metric.

\begin{definition}
\textbf{Inference Request} \\
% HK: This needs to be extended to support multi-modal models
The inference request $InfReq(\mu, IF_{i}(\mu))$ for a model $\mu$ on the i-th input frame for $\mu$, $IF_{i}(\mu)$, is defined as follows:
$$
InfReq(\mu, IF_{i}(\mu)) = (\mu, IF_{i}(\mu))
$$
\label{def:inference_request}
\end{definition}

Using~\autoref{def:inference_request}, we define the inference request time and deadline as follows.

\begin{definition}
\textbf{Inference Request time} \\
For an inference request $r = InfReq(\mu, F_{i}(inSrc))$, we define the inference request time $T_{req}(r)$ over an input stream $I$ as follows: 
$$
T_{req}(r) = L_{init}(inSrc) + i \times 1/SR(inSrc) \\ $$
$$
+ J_{t} \times 2 \times (Dist(inSrc, rand(i)) - 0.5)
$$

where $L_{init}(inSrc)$ indicates the setup latency of the input stream from the input source $inSrc$, $i \times 1/SR(inSrc)$ represents the time until reach the i-th frame under the streaming rate (FPS) of $SR(inSrc)$, and $J_{t} \times (Dist(inSrc, i)-0.5$ accounts for the impact of jitter on the arrival time modeled by a maximum jitter value $J_{t}$, a distribution $0 \leq Dist(inSrc, rand(i)) \leq 1$, and a deterministic random function $rand = f : \mathbb{N} \rightarrow \mathbb{R}$ . Note that we make the choice of $Dist(inSrc,rand(i))$ flexible for various scenarios. By default, $Dist(inSrc,rand(i))$ is a Gaussian distribution over $rand(i)$ value.

%where $I(r.\mu.src)$ refers to the element in $I$ whose $ID$ matches $r.\mu.src$ \textcolor{red}{vj:: i am a bit lost here on the $\mu$ and src -- is $\mu$ the model? it is hard to keep track of all the variables, so if we have the space maybe we can create a simple table with the symbol and definition} \HK{Thank you for the great suggestion; I love this idea. I'll create a table.}, and $Dist$ refers to a \textcolor{red}{what type of distribution is this? or do we just mean random value} \HK{I intentionally made this flexible. We can provide several functions to model different situations (e.g., we can adopt the Poisson distribution used for MLPerf)} distribution function that outputs a random value in $[0,1)$ following a specific distribution used to model random jitter.
\label{def:inference_request_time}
\end{definition}

Using a similar formulation, we define the inference deadline as follows.

\begin{definition}
\textbf{Inference Deadline} \\
For an inference request $r = infReq(\mu, IF_{i}(\mu))$ and $M(\mu) = (\mu, inSrc, ds, goal)$, we define the inference deadline $T_{dl}(r)$ over an input stream $I$ as follows: 
$$
T_{dl}(r) = L_{init}(inSrc) + (i + 1) \times 1/SR(inSrc) 
$$
using the same notation as~\autoref{def:inference_request_time}.
\label{def:deadline}
\end{definition}

Note that the deadline does not include the jitter term unlike the request time, which indicates that the system expects a certain processing rate even if there are jitters for the input data arrival time. Using the concepts defined so far, we define the inference-wise benchmark score next.

\subsection{Inference-wise Benchmark Score}
\label{sec:inference_wise_metric}

Because of the real-time processing nature of the Metaverse workloads, it is challenging to compare Metaverse device systems running real-time \abbrvWorkload{} using traditional metrics of using latency and energy. The latency measures the end-to-end execution time of each inference, which can be used to check if each model's deadlines are satisfied. However, achieving less latency than the deadlines does not offer benefits, making latency not an absolute minimization goal, unlike other ML systems targeting non-real-time \abbrvWorkload{}  workloads. In addition, we can adjust energy to meet the deadlines or optimize using the slack to the deadline (e.g., DVFS), which also makes energy a knob, not an absolute minimization target.

Therefore, we explore a new metric for \bench that considers all the unique aspects of real-time  \abbrvWorkload{}  workloads we discussed: (1) the task-specific deadlines based on usage scenarios, (2) end-to-end latency (i.e., how much latency does an ML system needs beyond the deadline?), (3) overall energy consumption, and (4) the quality of experience delivered. 

To facilitate an intuitive comparison of ML systems with many pillars, we propose a single metric score that captures all of the above. The single-score approach will also help motivate the industry to submit their evaluation results because the latency and energy can be confidential data that we cannot directly share with the public. Instead, the industry can offer the single score metric that captures overall performance on real-time and multi-model DL workloads to demonstrate the robust capabilities of their accelerator systems.

%To define such a metric, we define a cost function to be used to capture the relationship between the latency and deadlines.

To construct such a metric, we consider each aspect of real-time \abbrvWorkload{} workloads and model performance (e.g., accuracy, mIoU, and boxAP): real-time requirement, energy consumption, quality of experience, and model performance. We define a score for each pillar and combine them to define the single comprehensive metric. We define those score functions to be in [0, 1] range to facilitate component-wise analysis as well.

%\HK{Having a visualized example like one we had in the slides might be good. I'll first put all the contents and get back to this.}

To model real-time requirements, we consider the following observations: (1) Too much optimization on latency beyond the deadline does not lead to higher processing rates; even if a system finished the latency in only one cycle, the system still needs to wait for the next input frame. (2) reduced latency can still be helpful for scheduling other models. (3) violated deadline gradually damages the user experience (e.g., Achieving 59Hz for an eye-tracking model targeting 60Hz wouldn't significantly affect the user experience).

Based on those observations, we search for a function that (1) gradually rewards and penalizes the reduced and increased latency near a deadline (e.g., $\pm$ 0.5ms for a deadline of 10ms) and (2) outputs 0 and 1 if the latency is beyond or within the deadline. We discuss such a function in~\autoref{def:realtime_score_appendix}.

\begin{definition}
\textbf{Real-time requirement score} \\
For an inference request for the i-th input frame, $r = (\mu,IF_{i}(\mu))$, and the corresponding inference request time, $T_{req}(r)$ and deadline, $T_{dl}(r)$,
$$
RtScore(r) = \frac{1}{1+e^{k(Lat(r)-T_{slack}(r))}}
$$
where $Lat(r)$ represents the latency for the inference request $r$ and $T_{slack}(r) = T_{dl}(r) - T_{req}(r)$.
\label{def:realtime_score_appendix}
\end{definition}

%Inspired by the the Fermi-Dirac function\HK{TODO: add a citation or remove this},
We define the real-time requirement score $RtScore(t, T_{DL})$ in~\autoref{def:realtime_score_appendix}, where $t$ indicates the latency of the corresponding inference after the request. The score function can also be viewed as a modified Sigmoid function with shifting and scaling. A benefit of using $RtScore$ is that we can tune the constant $k$ depending on the deadline sensitivity. ~\autoref{fig:RealtimeScoreFunc} shows the change of the $RtScore$ based on the k value, and we can observe small $k$ values makes the function more sensitive around the deadline. We define k values based on the usage scenario and model in the benchmark suite. %\HK{TODO: define k values for each model in usage scenarios or claim that v0.1 will use the same values (e.g., k=15)}

\insertFigure{RealtimeScoreFunc}{An example real-time score function over different values of the parameter $k$ whose range is $[0,\infty)$. We assume the time window between the inference request time and deadline to be 1 ms in this example for simplicity.  If k is 0, the score is completely not relevant to the deadline (i.e., no sensitivity on deadline). If k is $\infty$, the score function becomes a piece-wise function that flips the score from 1 to 0 at the deadline.}

Using the real-time requirement score, we define overall score for an inference request as follows.

\begin{definition}
\textbf{Inference-wise score} \\
For an inference request on the j-th model $\mu_{j}$ in a usage scenario $\theta$ on the input frame $i$, $r(j,i) = (\mu,IF_{i}(\mu))$, we define a score for an inference request $S_{\theta}(r(j,i))$ as follows: 
$$
S_{\theta}(r(j,i)) = RtScore(r(j,i)) \times \frac{E_{max}-E^{(\mu_{j},i,h)}}{E_{max}} $$
$$
\times \frac{metric}{metric_{targ}} 
$$
%$$
%\times \frac{metric}{metric_{targ}} 
%$$
where 
$E_{max}$ refers to a large energy number an ML system shouldn't reach, used as an upper-bound value for the energy consumption. $E^{(\mu{j},i,h)}$ refers to the energy consumption for $r(j,i)$ on hardware $h$ (e.g., CPU, accelerator, and GPU). Note each of real-time, energy, and model performance scores is within the range of $[0,1]$, and the product of them is also within the range of $[0,1]$.
\label{def:inference_score}
\end{definition}

We extend the inference-wise score function to a benchmark score.

%\insertFigure{CostFunctions} {Three explored $CostScaleFn$ choices. For simplicity, we plot the functions with request time and deadline of 0 and 1 second, respectively.}

%\betterparagraph{Finding \latencycostfunction}
%If we find a good $CostScaleFn$ that reflects the real time requirements well, we obtain a good cost function $C_{\theta}(r(j,i))$. To define a good $CostScaleFn$, we make the following observations: 

%We explored three different functions for $CostScaleFn$ illustrated in~\autoref{fig:CostFunctions} : Dynamic Voltage and Frequency Scaling (DVFS), Fermi-Dirac (denoted as Fermi), and a piecewise function. \textcolor{red}{can we please explain why we pick these three to provide some intuitive rationale?}\HK{Thanks for the point. I'll enhance the following paragraphs to provide better rationale}


%\betterparagraph{DVFS} The first function models the typical dynamic voltage and frequency scale modes in silicon. DVFS function increases linearly until the deadline. After the deadline (1 second in the example in~\autoref{fig:CostFunctions}), the DVFS function quadratically increases until 1.5 seconds, reaching the maximum cost function value. This models the DVFS mode; higher energy can be used to bring the time back within real-time limits beyond the deadline.

%\betterparagraph{Fermi-Dirac Function} The second function is motivated by Fermi-Dirac function, which increases exponentially near the deadline to the maximum value. 

%\betterparagraph{Piecewise} The third function is a piecewise function, which is a step function that has the response at the deadline boundary.


%To understand the behavior of various $CostScaleFn$, we plot a score function assuming the score is the inverse of the cost (i.e., $score = \frac{1}{cost}$) in~\autoref{fig:logscore}. To observe the overall space of the score, we generate random data points with total latency between 1 milli-second and 1.5 seconds and energy between 0.1 and 1 Joule.

%\insertWideFigure{logscore} {The shape of initial score function when defined as $Score = \frac{1}{cost}$.}

%The score space in~\autoref{fig:logscore} is plotted in a log scale, and we observe that score is overly sensitive in the region with small latency and energy, which will result in significant score differences across good ML system designs (i.e., meets all the requirements) while minor score differences across good and ML system designs. As we expect the score provides a clear distinction between good and bad ML system designs, we revise the definition of the score function.

%\subsubsection{Scoring Function}
%\label{subsubsec:score_funciton}

%The high sensitivity at the lower end of values in~\autoref{fig:logscore} is based on our initial definition of the score as the inverse of the cost, which led to a $\frac{1}{x}$ curve. Although the high sensitivity of the score function is not desirable in the region with low latency and energy, it is desirable in the region with high latency and energy (e.g., dramatically reducing the score as the latency increases over deadline).

%Therefore, swap the sensitive region via by flipping the initial score function in the dimension of latency and energy pertaining to their maximum values: the maximum latency ($T_{DL} - T_{req}$) and a pre-defined large-enough energy value. This approach can be formluated as follows.

%\begin{definition}
%\textbf{Inference-wise Score Function} \\
%For each inference request $r(j,i) = R(\mu_{j},F_{i})$ where $(\mu_{j}, D_{j}, \gamma_{j}) \in \theta $, we define a score function $S_{\theta}(r(j,i))$ as follows: 

%$ S_{\theta}(r(j,i)) = $
%$$
%\sum_{i=1}^{|\theta|}{CostScaleFn(L_{max}^{(\mu_{j}, F_{i})} - L^{(\mu_{j}, F_{i})},T_{req}(r(j,i)), T_{DL}(r(j,i))}
%$$
%$$
%\times (E_{max} - E^{\theta{i}}) \times \omega_{i}.
%$$
%where $L_{max}{(\mu_{j}, F_{i})} = T_{DL}(r(j,i) - T_{req}(r(j,i))$

%\label{def:score_function}
%\end{definition}

%Note that $S'_{\Omega\}}$ replaces the latency($L^{\theta{i}}$) and energy ($E^{\theta{i}}$) with 1-$L^{\theta{i}}$ and $E_{max} - E^{\theta{i}}$, which flips the graph in latency and energy axes pertaining to 1 (second) and $E_{max}$ (J).

%\insertWideFigure{ScoreNegative2} {The shape of updated score functions defined in~\autoref{def:score_function}.}

%The shape of new score function is plotted in~\autoref{fig:ScoreNegative2}. It shows better behavior of the score function than the initial version plotted in~\autoref{fig:logscore} with reduced sensitivity with low latency/energy region. In particular, highly distinguished scores between low and high latency/energy regions reflects the real time requirements better. Based on the high delta near the deadline, we propose Fermi-Dirac function-based score for \bench.



\begin{definition}
\textbf{Usage-scenario Score} \\
Given time-out frames $targFrameID(j)$ for $inSrc(\mu_{j})$ (i.e., the number of frames to be processed for model j), we define the usage-scenario score $S_{\theta}$ as follows:

$$ S_{\theta} = \sum_{i=1}^{targFrameID(j)}{\sum_{j=1}^{|\theta|}}{S_{\theta}(r) \times \frac{N_{sat}}{N_{tot}}} 
$$
$$
\times \frac{100}{|targFrameID(j)| \times |\theta|}
$$
where $N_{tot}$ and $N_{sat}$ refer to the number of total inference requests and that of inference requests that satisfied deadlines.
\label{def:usage_scenario_score_function}
\end{definition}

Note that the latency information used in usage-scenario score reflect the delay due to previous inference requests. That is, if an inference request cannot launch until the next inference request on the same model due to other requests, the inference request should be dropped. To measure the impact of frame drop, the additional last term $\frac{N_{sat}}{N_{tot}}$ quantifies the portion of inferences that satisfied the deadlines. This is used as a measurement of the quality of user experience.

We divide the product of the sum of inference-wise score and the user experience score by the total number of frames that need to be processed ($targFrameID(j)$) and the number of models within the usage scenario $\theta$ to keep the overall range of the score metric within [0,1]. Finally, we multiply 100 to convert the range score into [0,100].

Using usage-scenario-wise scores, we define the overall score of \bench as the geometric-average of the scores for each usage scenario in \bench. 

\subsection{Schedule}

We do not propose a specific scheduler as it is a part of the ML system software to be evaluated. However we define valid schedules to satisfy the following conditions:

\begin{equation}
\forall h \in HW, \mu_{i} \in Dep_{\mu_{j}}, T_{end}(\mu_{i},h) < T_{start}(\mu_{j},h)
\label{eq:sched_dep}
\end{equation}

\begin{equation}
\begin{aligned}
\forall h \in HW, \forall (\mu, Dep_{\mu}, \gamma) \in \theta,  T_{start}(\mu_{i},h) \geq T_{end}(\mu_{j},h)
\end{aligned}
\label{eq:hw_occupancy}
\end{equation}

~\autoref{eq:sched_dep} indicates that the dependency order must be maintained in a schedule. ~\autoref{eq:hw_occupancy} illustrates that a hardware piece (e.g., a systolic array-based accelerator) cannot run two models simultaneously. That is, if a hardware module can run multiple models at the same time, the hardware module should be treated as multiple smaller hardware modules. This is to prevent potential confusion around the definition of a unit hardware module for running models.
%<Conditions>
%- Dependency order
%- Non-overlap within the same accelerator


==> tables/tab_applications.tex <==
\begin{table*}[t]
\centering
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{0pt}
\scriptsize
\caption{\small Selected example tasks and models in three MMMT applications.}
\label{tab:applications}  
\begin{tabular} {|@{~} l @{~}|l|l|c|}
\hline
\multicolumn{1}{|c|}{\textbf{Application}} &
\multicolumn{1}{c|}{\textbf{Selected Example Tasks}} &
\multicolumn{1}{c|}{\textbf{Example Model Type}} & 
\multicolumn{1}{c|}{\textbf{Real-time Processing}} \\
\hline

\multirow{4}{*}{Data Center~\cite{hazelwood2018applied}} 
   & User matching  & Support Vector Machine (SVM)~\cite{hazelwood2018applied} & \multirow{4}{*}{No} \\
   \cline{2-3}
   & Classification & Gradient-boosted Decision Tree (GBDT)~\cite{hazelwood2018applied} & \\   
   \cline{2-3}
   & Search & Multi-layer Perceptron (MLP)~\cite{hazelwood2018applied} & \\   
   \cline{2-3}
   & NLP & Recurrent Neural Network (RNN)~\cite{hazelwood2018applied} & \\
   \cline{2-3}
\hline
\multirow{4}{*}{Autonomous Driving~\cite{grigorescu2020survey}}
   & Steering Angle Control & Convolutional Neural Network (CNN) for Classification~\cite{bechtel2018deeppicar} & \multirow{4}{*}{Yes} \\   
   \cline{2-3}   
   & Driving Scene Understanding & Region-based CNN~\cite{he2017mask} & \\
   \cline{2-3}
   & 3D Object Detection & Point Cloud Network~\cite{qi2018frustum} & \\   
   \cline{2-3}
   & Visual Odometry (VO) & Ephemerality-aware visual odemetry~\cite{barnes2018driven} & \\   
   \cline{2-3}
\hline
\multirow{4}{*}{Virtual Reality~\cite{wu2019machine}} 
   & Hand Tracking & CNN for Segmentation~\cite{UNet} & \multirow{4}{*}{Yes} \\   
   \cline{2-3}
   & Image Processing & CNN~\cite{zhang2018shufflenet} & \\   
   \cline{2-3}
   & Pose Estimation & Mask R-CNN~\cite{he2017mask} & \\   
   \cline{2-3}
   & Action Segmentation & TCN~\cite{lea2017temporal} & \\   
   \cline{2-3}
\hline
 \end{tabular}
\end{table*}



==> tables/tab_benchmark_model_instances.tex <==
\begin{table*}[t]
\centering
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{0pt}
\scriptsize
\caption{\small }
\label{tab:benchmark_model_instances}
\begin{tabular} {|@{~} l @{~}|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{Task Category}} &
\multicolumn{1}{c|}{\textbf{Task}} &
\multicolumn{1}{c|}{\textbf{Reference}} &
\multicolumn{1}{c|}{\textbf{Model}} &
\multicolumn{1}{c|}{\textbf{Note}} 
\\
\hline

\hline
\multirow{6}{*}{\textbf{Interaction}} 
%    & Hand Tracking (HT) & Mask R-CNN~\cite{he2017mask} & \\
    & Hand Tracking (HT) & 
%    DLT~\cite{remelli2020lightweight} &
   Hand Shape/Pose~\cite{ge2019handshapepose} & 
   Hand Graph-CNN~\cite{handgraphcnn} &
   & 1/2 resolution \\ %Jason: with 3d pose supervision
    %Total Capture~\cite{joo2018total} \\
    
%    DLT with canonical fusion~\cite{remelli2020lightweight}  \\
    \cline{2-5}
%    & Pose Estimation (PE) & Interhand 2.6M~\cite{Interhand} & HT \\
%    \cline{2-5}
%    & Pose Estimation (PE) & Mask R-CNN~\cite{he2017mask} & ResNet-50-FPN (kp only)~\cite{he2017mask} &   \\
%    \cline{2-5}
    & Eye Segmentation (ES) & RITNet~\cite{chaudhary2019ritnet} & RITNet~\cite{RITNetCode} &  
    & 1/4 resolution \\
    \cline{2-5}
    & Gaze Estimation (GE) & Eyecod~\cite{you2022eyecod} & OpenEDS 2020~\cite{palmero2021openeds2020} 
    & 1/4 resolution \\
    \cline{2-5}
    & Keyword Detection (KD) & Key-Res-15~\cite{tang2018deep} & Google Speech Cmd~\cite{google_speech_commands} & \\
    \cline{2-5}
    & Automatic Speech Recognition (ASR) & Emformer ~\cite{shi2021emformer} & LibriSpeech~\cite{panayotov2015librispeech}  & \\
    \cline{2-5}
\hline
\multirow{5}{*}{\textbf{Context Understanding}} 
%    & Hand Tracking (HT) & Mask R-CNN~\cite{he2017mask} & \\
%    & Visual inertial odometry (VIO) & SOSNet~\cite{tian2019sosnet} & SoSNet32x32~\cite{SoSNet32x32} & UBC Phototour~\cite{brown2010discriminative} \\
%    \cline{2-5}
    & Semantic Segmentation (SS) & HRViT~\cite{gu2022multi} & HRViT-b1~\cite{HRViT-b1} & \\
    \cline{2-5}
%    & Object Classification (OC) & MNasNet~\cite{tan2019mnasnet} & MnasNet-A1(0.5x)~\cite{pytorch-mnasnet} & & \\
%    \cline{2-5}    
    & Object Detection (OD) & D2Go~\cite{d2go} & Faster-RCNN-FBNetV3A~\cite{Faster-RCNN-FBNetV3A} & \\
    \cline{2-5}
    & Action Segmentation (AS) & TCN ~\cite{lea2017temporal}  & ED-TCN~\cite{ED-TCN} & \\
    \cline{2-5}
    & Keyword Detection (KD) & Key-Res-15~\cite{tang2018deep} & res8-narrow~\cite{tang2018deep} & \\
    \cline{2-5}
    & Automatic Speech Recognition (ASR) & Emformer ~\cite{shi2021emformer} & EM-24L~\cite{shi2021emformer} & \\
    \cline{2-5}    
\hline
\multirow{3}{*}{\textbf{World Locking}}
    & Depth Estimation (DE) & MiDaS~\cite{ranftl2020towards} & midas\_v21\_small~\cite{midasV21Small} & \\
    \cline{2-5}
%    & Stereo Depth Estimation (StDE) & HITNet~\cite{tankovich2021hitnet} & HITNet~\cite{tankovich2021hitnet} & KITTI~\cite{geiger2012we}\\
%    \cline{2-5}
    & Depth Refinement (DR) & Sparse-to-Dense~\cite{ma2018sparse} & RGBd-200~\cite{ma2018sparse} for KITTI & \\
    \cline{2-5}
    & Plane Detection (PD) & PlaneRCNN~\cite{liu2019planercnn} & PlaneRCNN~\cite{liu2019planercnn} & 1/4 resolution \\ % ScanNet~\cite{dai2017scannet} \\
    \cline{2-5}
\hline
\end{tabular}
\end{table*}

% ML Op list + interesting properties + implication to the architecture 

% Diagram that shows the full dependency graphs for a usage scenario

% Accuracy target for individual model vs entire pipeline

% Why the metric is good enough 



==> tables/tab_benchmark_models.tex <==
\begin{table*}[t]
\centering
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{0pt}
\scriptsize
\caption{\small Unit tasks in Metaverse applications and proxy unit models for each task. The Reference column lists the papers that introduced the model architectures. We provide a list of model instances from the model architectures used for \bench  in~\autoref{tab:benchmark_model_instances}. The dataset column indicates the dataset to be used for each model. Note that some models (e.g., KD) are used for multiple task categories. For some models, we down-scale the input resolution to adjust the models to the context of wearable/mobile devices.}
\label{tab:benchmark_models}
\begin{tabular} {|@{~} l @{~}|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{Task Category}} &
\multicolumn{1}{c|}{\textbf{Task}} &
\multicolumn{1}{c|}{\textbf{Reference}} &
\multicolumn{1}{c|}{\textbf{Dataset}} &
\multicolumn{1}{c|}{\textbf{Note}} 
\\
\hline

\hline
\multirow{5}{*}{\textbf{Interaction}} 
%    & Hand Tracking (HT) & Mask R-CNN~\cite{he2017mask} & \\
    & Hand Tracking (HT) & 
%    DLT~\cite{remelli2020lightweight} &
   Hand Shape/Pose~\cite{ge2019handshapepose} & 
   Stereo Hand Pose~\cite{stereohandpose}
   & 1/2 resolution \\ %Jason: with 3d pose supervision
    %Total Capture~\cite{joo2018total} \\
    
%    DLT with canonical fusion~\cite{remelli2020lightweight}  \\
    \cline{2-5}
%    & Pose Estimation (PE) & Interhand 2.6M~\cite{Interhand} & HT \\
%    \cline{2-5}
%    & Pose Estimation (PE) & Mask R-CNN~\cite{he2017mask} & ResNet-50-FPN (kp only)~\cite{he2017mask} &   \\
%    \cline{2-5}
    & Eye Segmentation (ES) & RITNet~\cite{chaudhary2019ritnet} & OpenEDS 2019~\cite{garbin2019openeds} 
    & 1/4 resolution \\
    \cline{2-5}
    & Gaze Estimation (GE) & Eyecod~\cite{you2022eyecod} & OpenEDS 2020~\cite{palmero2021openeds2020} 
    & 1/4 resolution \\
    \cline{2-5}
    & Keyword Detection (KD) & Key-Res-15~\cite{tang2018deep} & Google Speech Cmd~\cite{google_speech_commands} & \\
    \cline{2-5}
    & Automatic Speech Recognition (ASR) & Emformer ~\cite{shi2021emformer} & LibriSpeech~\cite{panayotov2015librispeech}  & \\
    \cline{2-5}
\hline
\multirow{5}{*}{\textbf{Context Understanding}} 
%    & Hand Tracking (HT) & Mask R-CNN~\cite{he2017mask} & \\
%    & Visual inertial odometry (VIO) & SOSNet~\cite{tian2019sosnet} & SoSNet32x32~\cite{SoSNet32x32} & UBC Phototour~\cite{brown2010discriminative} \\
%    \cline{2-5}
    & Semantic Segmentation (SS) & HRViT~\cite{gu2022multi} & Cityscape~\cite{cordts2016cityscapes} 
    & \\
    \cline{2-5}
%    & Object Classification (OC) & MNasNet~\cite{tan2019mnasnet} & MnasNet-A1(0.5x)~\cite{pytorch-mnasnet} & & \\
%    \cline{2-5}    
    & Object Detection (OD) & D2Go~\cite{d2go} & COCO~\cite{lin2014microsoft} 
    & \\
    \cline{2-5}
    & Action Segmentation (AS) & TCN ~\cite{lea2017temporal} & GTEA~\cite{fathi2011learning} 
    & \\
    \cline{2-5}
    & Keyword Detection (KD) & Key-Res-15~\cite{tang2018deep} & Google Speech Cmd~\cite{google_speech_commands} 
    & \\
    \cline{2-5}
    & Automatic Speech Recognition (ASR) & Emformer ~\cite{shi2021emformer} & LibriSpeech~\cite{panayotov2015librispeech} 
    & \\
    \cline{2-5}    
\hline
\multirow{3}{*}{\textbf{World Locking}}
    & Depth Estimation (DE) & MiDaS~\cite{ranftl2020towards} & KITTI~\cite{geiger2012we}
    & \\
    \cline{2-5}
%    & Stereo Depth Estimation (StDE) & HITNet~\cite{tankovich2021hitnet} & HITNet~\cite{tankovich2021hitnet} & KITTI~\cite{geiger2012we}\\
%    \cline{2-5}
    & Depth Refinement (DR) & Sparse-to-Dense~\cite{ma2018sparse} & KITTI~\cite{geiger2012we}
    & \\
    \cline{2-5}
    & Plane Detection (PD) & PlaneRCNN~\cite{liu2019planercnn} &
    KITTI~\cite{geiger2012we}
    & 1/4 resolution \\ % ScanNet~\cite{dai2017scannet} \\
    \cline{2-5}
\hline
\end{tabular}
\end{table*}

% ML Op list + interesting properties + implication to the architecture 

% Diagram that shows the full dependency graphs for a usage scenario

% Accuracy target for individual model vs entire pipeline

% Why the metric is good enough 


